Strike (with) a Pose: Neural Networks Are Easily Fooled by Strange Poses of Familiar Objects

Despite excellent performance on stationary test sets, deep neural networks (DNNs) can fail to generalize to out-of-distribution (OoD) inputs, including natural, non-adversarial ones, which are common in real-world settings. In this paper, we present a framework for discovering DNN failures that harnesses 3D renderers and 3D models. That is, we estimate the parameters of a 3D renderer that cause a target DNN to misbehave in response to the rendered image. Using our framework and a self-assembled dataset of 3D objects, we investigate the vulnerability of DNNs to OoD poses of well-known objects in ImageNet. For objects that are readily recognized by DNNs in their canonical poses, DNNs incorrectly classify 97% of their pose space. In addition, DNNs are highly sensitive to slight pose perturbations. Importantly, adversarial poses transfer across models and datasets. We find that 99.9% and 99.4% of the poses misclassified by Inception-v3 also transfer to the AlexNet and ResNet-50 image classifiers trained on the same ImageNet dataset, respectively, and 75.5% transfer to the YOLOv3 object detector trained on MS COCO.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.8	//
$z_ delta	paper.tex	/^\\subsection{$z_{\\delta}$-constrained random search}$/;"	b
3D Transformation Matrix	paper.tex	/^\\section{3D Transformation Matrix}\\label{sec:trans-mat}$/;"	s
3D object dataset	paper.tex	/^\\subsection{3D object dataset}$/;"	b
3D renderers	paper.tex	/^\\subsection{3D renderers}$/;"	b
Background images	paper.tex	/^\\subsection{Background images}$/;"	b
Classification networks	paper.tex	/^\\subsection{Classification networks}$/;"	b
Construction	paper.tex	/^\\subsection{Construction}\\label{sec:construction}$/;"	b
Correct classifications are highly localized in the rotation and translation parameter landscape	paper.tex	/^\\subsection{Correct classifications are highly localized in the rotation and translation parameter landscape}$/;"	b
Discussion and Conclusion	paper.tex	/^\\section{Discussion and Conclusion}$/;"	s
Evaluation	paper.tex	/^\\subsection{Evaluation}\\label{sec:evaluation}$/;"	b
Experiment Setup on Differentiable renderer	paper.tex	/^\\section{Experiment Setup on Differentiable renderer}\\label{sec:dr-expr}$/;"	s
Experiments and Results	paper.tex	/^\\section{Experiments and Results}$/;"	s
Extended description of the 3D object dataset and its evaluation	paper.tex	/^\\section{Extended description of the 3D object dataset and its evaluation}$/;"	s
Generalization on adversarial examples with non empty background	paper.tex	/^\\section{Generalization on adversarial examples with non-empty background}$/;"	s
Gradient descent with DR approximated gradients	paper.tex	/^\\section{Gradient descent with DR-approximated gradients}\\label{sec:kr}$/;"	s
Gradient descent with finite difference	paper.tex	/^\\subsection{Gradient descent with finite-difference}$/;"	b
Methods	paper.tex	/^\\section{Methods}$/;"	s
Multi camera Optimization	paper.tex	/^\\subsection{Multi-camera Optimization}%$/;"	b
Neural networks are easily confused by object rotations and translations	paper.tex	/^\\subsection{Neural networks are easily confused by object rotations and translations}$/;"	b
Notes on optimization speed between using differentiable renderer and non differentiable renderer	paper.tex	/^\\section{Notes on optimization speed between using differentiable renderer and non-differentiable renderer}$/;"	s
Parameter augmentation	paper.tex	/^\\subsection{Parameter augmentation}%$/;"	b
Pipeline	paper.tex	/^\\section{Pipeline}$/;"	s
Pose transformations	paper.tex	/^\\subsection{Pose transformations}$/;"	b
Problem formulation	paper.tex	/^\\subsection{Problem formulation}$/;"	b
Random search	paper.tex	/^\\subsection{Random search}$/;"	b
Related work	paper.tex	/^\\section{Related work}$/;"	s
T SNE plot of images generated from 3D objects	paper.tex	/^\\section{T-SNE plot of images generated from 3D objects}$/;"	s
Transferability from Inception v3 to YOLO v3	paper.tex	/^\\section{Transferability from Inception v3 to YOLO v3}$/;"	s
Verification of OoD examples are not found in the ImageNet training set	paper.tex	/^\\section{Verification of OoD examples are not found in the ImageNet training set}\\label{sec:nearest_neighbors}$/;"	s

